Magicremover: Tuning-free Text-guided Image inpainting with Diffusion Models

Image inpainting aims to fill in the missing pixels with visually coherent and semantically plausible content. Despite the great progress brought from deep generative models, this task still suffers from i. the difficulties in large-scale realistic data collection and costly model training; and ii. the intrinsic limitations in the traditionally user-defined binary masks on objects with unclear boundaries or transparent texture. In this paper, we propose MagicRemover, a tuning-free method that leverages the powerful diffusion models for text-guided image inpainting. We introduce an attention guidance strategy to constrain the sampling process of diffusion models, enabling the erasing of instructed areas and the restoration of occluded content. We further propose a classifier optimization algorithm to facilitate the denoising stability within less sampling steps. Extensive comparisons are conducted among our MagicRemover and state-of-the-art methods including quantitative evaluation and user study, demonstrating the significant improvement of MagicRemover on high-quality image inpainting. We will release our code at https://github.com/exisas/Magicremover.

==> subsections/introduction.tex <==
\section{Introduction}
Image Inpainting is a prominent research area in computer vision, which focuses on the restoration and completion of images by filling in missing or corrupted regions with plausible and visually coherent content. These restored areas need to be consistent with the rest of the image and semantically reasonable, necessitating inpainting methods to have robust generative capabilities. In recent years, with the rapid development of generative models such as GANs \citep{goodfellow2020generative} and diffusion models \citep{ho2020denoising}, image inpainting tasks have made significant strides.
Although existing image inpainting methods, such as RePaint \citep{lugmayr2022repaint} and LaMa \citep{suvorov2021resolution}, can successfully restore large areas of arbitrary shapes and even fill in mask areas with content matching textual descriptions, like Imagen editor \citep{wang2023imagen} and SmartBrush \citep{xie2023smartbrush}, they still require fine annotations for each mask, which is inconvenient for users, especially when the mask does not have obvious boundaries such as soft shadow. In contrast, our work attempts to use text to annotate the areas intended for inpainting. Moreover, existing image inpainting methods utilize a binary mask, which erases all information within the mask area during the inpainting process. This is highly unfavorable for semi-transparent object images, such as shadow, light, reflection, etc. For example, current inpainting methods are unable to preserve the information of leaves under the light source while removing the light source itself as shown in Figure \ref{front}(c).


The aforementioned two challenges, whether using text to erase areas of interest or erasing semi-transparent objects while preserving background details, are extremely demanding. Fortunately, with the rapid development of generative models, a variety of large-scale text-to-image models have emerged in recent years, such as Stable Diffusion \citep{rombach2022high}, Imagen \citep{saharia2022photorealistic}, and Dalle2 \citep{ramesh2022hierarchical}. These models possess multimodal capabilities that lay the foundation for establishing connections between text and areas of interest. For example, Prompt2Prompt \citep{hertz2022prompt} is built based on the correspondence between intermediate text and the features of generated images. They found that the cross-attention map could provide the spatial response of each word in the image, which can be used as a medium for editing images. In addition, these text-to-image models are trained on vast amounts of paired text-image datasets, providing them with a certain level of image understanding and text comprehension capabilities, which in turn offer the potential for training-free, layered object erasure.

To address the aforementioned problems, we propose Magic Eraser: a text-driven, mask-free image inpainting algorithm capable of erasing semi-transparent objects. Our method requires no additional training and can be directly applied to pre-trained text-to-image models. 
% Specifically, we employ a null-text inversion \citep{mokady2023null} approach to reconstruct images based on the input textual conditions. Through this step, we can obtain the spatial response of each word in the input text from the cross-attention map of the real image. 
Specifically, we first perform image inversion and obtain the spatial response of each word from the cross-attention map of the original image by null-text inversion \citep{mokady2023null}.
Subsequently, we convert the object removal signal into gradients along with classifier guidance \citep{dhariwal2021diffusion}, allowing for the gradual removal of objects during the sampling process. 
Moreover, in order to further reduce the time cost, we propose a novel classifier optimization method to reduce the inversion steps while enhancing the editing capabilities and stability.
% We demonstrate our method on the Stable Diffusion ... and SDXL ... but can also be applied to other text-to-image pretrained models?

Our main contributions are summarized as follows:

\begin{itemize}
  \item [1.] 
    We develop an inpainting algorithm that erases objects solely through text without the need for masks, by using only pre-trained Stable Diffusion models and without requiring any additional tuning.
   % We develop an inpainting algorithm that erases objects solely through text without the need for masks, by employing pre-trained Stable Diffusion models without any additional training.
  \item [2.]
    To the best of our knowledge, our method is the first to employ a diffusion model to achieve the erasure of semi-transparent objects such as light and shadow, while simultaneously preserving the background information behind these transparent objects.
  \item [3.]
    We propose a diffusion model-agnostic optimization sampling algorithm that enhances the capabilities and stability of classifier guidance conditional sampling.  
\end{itemize}



==> subsections/method.tex <==
\section{Method}
\label{sec:method}
\begin{figure*}[h]
\centering
\includegraphics[width=\linewidth]{method.pdf}
\caption{Framework overview. We first invert the input image to obtain the noisy latent $\mathbf{z}_t$ at the t-th time step and optimize a set of null text embedding lists for image reconstruction. Next, we utilize the inversion results to generate the edited image under the guidance of attention. During the editing process, cross-attention mechanisms are employed to obtain optimized image guidance, while self-attention mechanisms are utilized to ensure similarity with the original image.
}
\label{architecture}
\end{figure*}

\subsection{overview}
\label{method:overview}
Unlike traditional inpainting tasks, our goal is to erase objects described by text, rather than those marked by masks. To address this issue, we propose a simple and efficient method called Magic Eraser, which uses the publicly available text-to-image generative model to edit images in a training-free manner. Our method consists of three parts: an image inversion module to achieve text-image alignment, an attention guidance module to implement object erasure and background preservation, and a classifier optimization module to enhance the editing capability and stability of the algorithm. The overview of our method is presented in Fig.\ref{architecture}.

\subsection{Text-image alignment}
\label{method:text-image alignment}
The image inversion module requires users to provide an image and its corresponding text description. The text description can range from a single word describing the object to be erased to a detailed description containing the target object and other information about the image. The purpose of text-image alignment is to enable the model to reconstruct the image based on the given text and initial noise so that it can provide a more accurate spatial response for the target word during the denoising process. DDIM inversion + DDIM denoising is a commonly used method for text-image alignment. Although it can preserve most of the image information, it inevitably causes some visible detail loss. Therefore, we adopt a more advanced approach called Null-text inversion \citep{mokady2023null}, which taking the DDIM inversion trajectory $\left\{\mathbf{z}_t^{\mathrm{inv}}\right\}_{t=1}^T$ and the source prompt $\mathbf{y}$ as input, and then optimizes a set of null-text embeddings $\left\{\varnothing_t\right\}_{t=1}^T$ according to the following equation:
\begin{equation}
\min _{\varnothing_t}\left\|\mathbf{z}_{t-1}^{\mathrm{inv}}-f_\theta\left(\mathbf{z}_t, t, \mathbf{y} ; \varnothing_t\right)\right\|_2^2,
\label{null-text}
\end{equation}
where $f_\theta$ represents applying DDIM sampling on the noise predicted by the pre-trained image diffusion model $\epsilon_\theta(\mathbf{x}_t ; t, \mathbf{y}) $.

\subsection{Attention guidance}
\label{sec_atten_guid}
In our approach, we leverage the cross-attention module within the neural network $\epsilon_\theta\left(\mathbf{z}_t ; t, \mathbf{y}\right)$ to obtain guidance for erasing objects. Specifically, For any word with index $k$ in a given text condition $\mathbf{y}$, we are able to obtain its corresponding softmax-normalized attention matrices $\mathcal{A}_{t, k} \in \mathbb{R}^{H \times W}$ at any timestep $t$. This cross-attention map can be regarded as the spatial response of the image to that specific word. Therefore, optimizing $\mathbf{z}_t$ towards the direction where the response to the $k$-th word is zero naturally leads to the erasure of the object corresponding to the $k$-th word.
Unfortunately, the cross-attention map corresponding to each word not only contains the spatial response to that word but also includes some responses from other objects in the image. Directly optimizing $z_t$ towards the direction of zero response may cause significant changes in the image background. To overcome this issue, we propose three improvements. 
\paragraph{Relaxing constraints.} We optimize $\mathbf{z}_t$ towards a lower response direction rather than an absolute zero matrix. Since the pixel values in the cross-attention map $\mathcal{A}_{t, k}$ represent the degree of relevance to the corresponding word, generally, the values in $\mathcal{A}_{t, k}$ from high to low correspond to the target object, shadows (reflection, etc. if present), and the background. Therefore, we set the optimization target as a matrix filled with pixel values corresponding to the bottom $10\%$ of the values in the cross-attention map. Empirically, we find that setting the optimization target in this way is sufficient to completely erase the target object. In addition, to satisfy users' desire to erase objects while preserving features like shadows, we provide a hyperparameter $\lambda \in [0,1] $ to control the degree of object erasure. Therefore, the guidance for erasing the object corresponding to the $k$-th word at timestep $t$ can be defined as follows:
\begin{equation}
\label{guidance}
g(t,k,\lambda)= \| \mathcal{A}_{t, k} - [\min(\mathcal{A}_{t, k}) + \lambda (\max(\mathcal{A}_{t, k}) -\min(\mathcal{A}_{t, k}))] \mathcal{A}_{t, k}\|_1.
\end{equation}

\paragraph{Reweight perturbation.} Since the areas with higher relevance to their corresponding word in the cross-attention map have larger values, and those with lower relevance have smaller values, directly multiplying it with the additive perturbation of the classifier guidance can greatly suppress background changes. Therefore, for erasing a single object corresponding to a word, our attention guidance classifier sampling method can be written as:
\begin{equation}
\label{attention guidance}
\hat{\epsilon}^{guid}_t=(1+s) \epsilon_\theta\left(\mathbf{z}_t ; t, \mathbf{y}\right)-s \epsilon_\theta\left(\mathbf{z}_t ; t, \varnothing\right)+\mathcal{A}_{t, k} \odot \nabla_{\mathbf{z}_t} g(t,k,\lambda)
\end{equation}

In some cases, such as removing a specific color of vehicles from an image containing cars of different colors, or erasing both people and trees from a image, processing with a single cross-attention map for one word cannot meet the requirements. To further expand the applicability of our method, we make some modifications to Eq.\ref{attention guidance}. When we want to erase $m$ different categories of objects, each described by $n$ words, we change it to the following form:
\begin{equation}
\label{attention guidance fin}
\hat{\epsilon}^{guid}_t=(1+s) \epsilon_\theta\left(\mathbf{z}_t ; t, \mathbf{y}\right)-s \epsilon_\theta\left(\mathbf{z}_t ; t, \varnothing\right)+ (\sum_{m} \prod_{n} \mathcal{A}_{t, k}) \odot (\nabla_{\mathbf{z}_t} \sum_{m \times n} g(t,k,\lambda))
\end{equation}

Additionally, our method supports the use of an extra input mask $M$\footnote{Unless specifically stated, the results presented in this paper are achieved without masks.} to label instances in certain extreme cases, such as when there are multiple objects of the same category in an image, making it more difficult to describe the desired instance to erase than obtaining a mask. In this situation, we only need to add an additional term $\nabla_{\mathbf{z}_t} (\hat{\mathbf{z}}_{t-1} - \mathbf{z}^{inv}_{t-1}) \odot (1-M)$ to Eq.\ref{attention guidance fin}.

\paragraph{Self-attention guidance.} Inspired by the consistency in video editing works \citep{khachatryan2023text2video,wang2023zero}, self-attention plays a vital role in preserving information such as image texture and color. In order to further maintain the similarity between the edited image and the original image, we preserve the $\mathbf{K}$ matrix and $\mathbf{V}$ matrix of the self-attention module during the reconstruction process, and modify the self-attention module during the editing process as follows:
\begin{equation}
\operatorname{Attention}(\mathbf{Q}_{edit}, \mathbf{K}_{rec}, \mathbf{V}_{rec})=\operatorname{softmax}\left(\frac{\mathbf{Q}_{edit} \mathbf{K}_{rec}^T}{\sqrt{d}}\right) \mathbf{V}_{rec}
\end{equation}

\subsection{classifier Optimization}

\begin{figure}[ht]
\begin{subfigure}{.42\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{ddim_sampling.png}  
  \caption{DDIM sampling}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.58\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{opt_sampling.png}  
  \caption{Ours}
  \label{fig:sub-second}
\end{subfigure}
\caption{Illustration of Classifier optimization. Our classifier optimization operation can be performed any number of times at any given sampling moment $t$.}
\label{fig:fig}
\end{figure}

In Sec.\ref{method:text-image alignment}, we use Null-text inversion \citep{mokady2023null} to achieve image and text alignment, which requires optimizing Eq.\ref{null-text} for about 100 steps at each sampling moment. Therefore, the more sampling steps we use, the more steps Null-text inversion optimization takes, which is time-consuming. To reduce time while not compromising the editing capability of the algorithm, we propose the classifier optimization operation in this section. Considering that in diffusion-based image editing methods, besides adding perturbations to the predicted noise like classifier guidance sampling, we can also optimize the noisy latent $\mathbf{z}_t$ using gradient descent algorithms through an optimizer \citep{shi2023dragdiffusion}. Given the similarities between these two approaches, we attempt to make some modifications to classifier guidance to achieve the same function as the optimizer, optimizing $\mathbf{z}_t$ without changing $t$. This allows us to increase the optimization steps, reduce the number of sampling steps, and ultimately decrease the time required for null-text inversion.

%In diffusion-based methods, to edit images, either optimize the noisy latent $\mathbf{z}_t$ through an optimizer \citep{shi2023dragdiffusion}, or modify the predicted noise in the reverse process through classifier guidance sampling \citep{epstein2023diffusion}. The diffusion model generates images in the order of layout-content-texture. Due to the limitations of computational resources, optimizing noisy latent $\mathbf{z}_t$ with an optimizer cannot optimize the noisy latents at all times, so it is impossible to edit attributes like layout, content and texture simultaneously. Although the classifier sampling method can adjust the latent at any point during the sampling process, the limited number of sampling steps prevents sufficient adjustment of each attribute. Therefore, this section makes a modification to the classifier sampling method, improving the image adjustment capability of classifier sampling without increasing $T$ (the number of time steps).


Let us reconsider Eq.\ref{ddim}, as DDIM can be implemented in the order of first predicting inital latent $\mathbf{z}_0$ from noisy latent $\mathbf{z}_t$ and then adding noise to $\mathbf{z}_{t-1}$. In order to update $\mathbf{z}_t$ an unlimited number of times without increasing $T$, we try to add an optimization step in the denoising process, that is, modifying DDIM to predict $\mathbf{z}_0$ from $\mathbf{z}_t$, and then add noise to $\mathbf{z}^{opt}_t$:
\begin{equation}
\begin{aligned}
\mathbf{z}^{opt}_{t}=\sqrt{\alpha_{t}} \left(\frac{\mathbf{z}_t-\sqrt{1-\alpha_t} \hat{\epsilon}^{guid}_t\left(\mathbf{z}_t\right)}{\sqrt{\alpha_t}}\right) +\sqrt{1-\alpha_{t}-\sigma_t^2} \cdot \hat{\epsilon}^{guid}_t\left(\mathbf{z}_t\right) +\sigma_t \epsilon_t
\end{aligned}
\end{equation}
To guarantee the resemblance between the edited image and the original image, as well as to regulate the randomness during the sampling process, it is beneficial to set $\sigma_t$ to 0. However, this may result in $\mathbf{x}^{opt}_t$ being exactly equal to $\mathbf{x}_t$, which would not serve the purpose of updating $x_t$. Therefore, we replace the noise used in the "predicted $\mathbf{x}_0$" and the "direction pointing to $\mathbf{x}_t$" process with two different noise sources:
\begin{equation}
\begin{aligned}
\mathbf{z}^{opt}_{t}&=\sqrt{\alpha_{t}} \left(\frac{\mathbf{z}_t-\sqrt{1-\alpha_t} \hat{\epsilon}_t\left(\mathbf{z}_t\right)}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t}} \cdot \hat{\epsilon}^{guid}_t\left(\mathbf{z}_t\right) 
\end{aligned}
\end{equation}

where $\hat{\epsilon}_t=(1+s) \epsilon_\theta\left(\mathbf{x}_t ; t, y\right)-s \epsilon_\theta\left(\mathbf{x}_t ; t, \varnothing\right)$ refers to the noise predicted through classifier-free guidance approach. The proposed optimization step can be integrated into the denoising process at any given time t, allowing for the arbitrary updates of $\mathbf{x}_t$ without being restricted by the limitation that the sampling steps should be less than T. 
In our experiments, we found that during the denoising process, using the noise before perturbation $\hat{\epsilon}_t$ for "predicted $\mathbf{x}_0$" and the noise after perturbation $\hat{\epsilon}'_t$ for "direction pointing to $\mathbf{x}_t$" can also improve the editing results, which has been confirmed in the image editing method by \cite{kwon2022diffusion}. Detail of our final sampling process can be found in Algorithm \ref{sampling}.

\begin{algorithm}[!h]
    \caption{sampling algorithm}
    \label{sampling}
    \textbf{Parameter}: Initialize model $\sim \epsilon_\theta$.  \\
        Input image $\mathbf{x}_0$ \\
        Input caption $\mathbf{y}$  \\
        Number of diffusion steps $T$. \\
        optimization time list opt\_t. \\
        
    \begin{algorithmic}[1] %[1] enables line numbers
      \State  $\mathbf{z}_0=\mathcal{E}(\mathbf{x}_0)$
      \State  $\left\{\mathbf{z}_t^{\text {inv }}\right\}_{t=1}^T=DDIM-inversion\left(\mathbf{z}_0\right)$
      \State  $\{\varnothing_t\}_{t=1}^T=Null-text-optimization\left(\left\{\mathbf{z}_t^{\text {inv }}\right\}_{t=1}^T, \mathbf{y}\right)$ 
      \For{t in scheduler.timesteps}
        \State $\hat{\epsilon}_t=(1+s) \epsilon_\theta\left(\mathbf{x}_t ; t, y\right)-s \epsilon_\theta\left(\mathbf{x}_t ; t, \varnothing\right)$
        \State $\hat{\epsilon}^{guid}_t=\hat{\epsilon}_t+ \sum_{m} \prod_{n} \mathcal{A}_{t, k} \nabla_{\mathbf{z}_t} \sum_{m \times n} g(t,k,\lambda)$
        \State $\mathbf{z}^{opt}_{t}=\mathbf{z}_{t}$

        \If{t in opt\_t}
            \For{i in range(len(opt\_t))}
                \State $\mathbf{z}^{opt}_{t}=\sqrt{\alpha_{t}} \left(\frac{\mathbf{z}_t-\sqrt{1-\alpha_t} \hat{\epsilon}_t\left(\mathbf{z}_t\right)}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t}} \cdot \hat{\epsilon}^{guid}_t\left(\mathbf{z}_t\right) $
            \EndFor
        \EndIf
        
        \State $\mathbf{z}_{t-1}=\sqrt{\alpha_{t-1}} \left(\frac{\mathbf{z}^{opt}_t-\sqrt{1-\alpha_t} \hat{\epsilon}_t\left(\mathbf{z}^{opt}_t\right)}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t-1}} \cdot \hat{\epsilon}^{guid}_t\left(\mathbf{z}^{opt}_t\right) $
      \EndFor
    
    \end{algorithmic}
\end{algorithm}

\iffalse
\begin{equation}
\begin{aligned}
\mathbf{x}_{t-1}&=\sqrt{\alpha_{t-1}} \left(\frac{\mathbf{x}_t-\sqrt{1-\alpha_t} \hat{\epsilon}'_t\left(\mathbf{x}_t\right)}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t-1}-\sigma_t^2} \cdot \hat{\epsilon}'_t\left(\mathbf{x}_t\right) +\sigma_t \epsilon_t
\end{aligned}
\end{equation}


\begin{equation}
\begin{aligned}
\mathbf{x}_{t-1}&=\sqrt{\alpha_{t-1}} \left(\frac{\mathbf{x}_t-\sqrt{1-\alpha_t} \hat{\epsilon}_t\left(\mathbf{x}_t\right)}{\sqrt{\alpha_t}}\right)+\sqrt{1-\alpha_{t-1}-\sigma_t^2} \cdot \hat{\epsilon}'_t\left(\mathbf{x}_t\right) +\sigma_t \epsilon_t
\end{aligned}
\end{equation}
\fi



==> subsections/relatedwork.tex <==
\section{Related Work}
\subsection{Diffusion Models}
\zl{simplify this section, remove some equations that are not used in sec.3}
Recently, Diffusion Probabilistic Models (DPMs)~\citep{ho2020denoising,song2020score} have received increasing attention due to their impressive ability in image generation. It has broken the long-term domination of GANs \citep{goodfellow2020generative} and become the new state-of-the-art protocol in many computer vision tasks.
%It has broken the long-term domination of GANs and become the new state-of-the-art protocol in many computer vision tasks, such as image/video/3D synthesis~\citep{dhariwal2021diffusion,saharia2022photorealistic,ramesh2022hierarchical,nichol2021glide}, image inpainting~\citep{lugmayr2022repaint} and super-resolution \citep{rombach2022high}. 
DPMs can be divided into forward and reverse processes. Given a sample from data distribution $\mathbf{x}_0 \sim p_{data}(\mathbf{x})$, the forward process gradually destroys the structure in data by adding Gaussian noise to $x_0$ for $T$ steps, according to the variance schedule $\beta_1,...,\beta_T$:
\begin{equation}
\begin{aligned}
%q\left(\mathbf{x}_{1: T}\right) & =\prod_{t=1}^T q\left(\mathbf{x}_t \mid \mathbf{x}_{t-1}\right) \\
q\left(\mathbf{x}_t \mid \mathbf{x}_{t-1}\right) & =\mathcal{N}\left(\mathbf{x}_t ; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I}\right).
\end{aligned}
\end{equation}
Subsequently, a U-Net \citep{ronneberger2015u} can be trained  to predict the noise added during the forward process $\epsilon_\theta\left(\mathbf{x}_t; t \right)$ based on the given condition $\mathbf{y}$ with loss:
\begin{equation}
L(\theta)=\mathbb{E}_{t \sim \mathcal{U}(1, T), \epsilon_t \sim \mathcal{N}(0, \mathbf{I})}\left[w(t)\left\|\epsilon_t-\epsilon_\theta\left(\mathbf{x}_t ; t, \mathbf{y}\right)\right\|^2\right],
\end{equation}
where the condition $\mathbf{y}$ can be $\varnothing$, text \citep{rombach2022high} or images \citep{ho2022cascaded}, etc.

After the training is completed, the reverse process can trace back from the isotropic Gaussian noise $\mathbf{x}_T \sim$ $\mathcal{N}\left(\mathbf{x}_T ; \mathbf{0}, \mathbf{I}\right)$ to the initial data distribution using the predicted noise,
\begin{align}
\hat{\mathbf{x}}_0 =\frac{1}{\sqrt{\bar{\alpha}_t}}\left(\mathbf{x}_t-\sqrt{1-\bar{\alpha}_t} \epsilon_\theta\left(\mathbf{x}_t ; t, \mathbf{y}\right) \right) \\
p\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t, \hat{\mathbf{x}}_0\right)=\mathcal{N}\left(\mathbf{x}_{t-1} ; \tilde{\boldsymbol{\mu}}_t\left(\mathbf{x}_t, \hat{\mathbf{x}}_0\right), \tilde{\beta}_t \mathbf{I}\right) \label{reverse},
\end{align}

where $ \tilde{\boldsymbol{\mu}}_t\left(\mathbf{x}_t, \hat{\mathbf{x}}_0\right):=\frac{\sqrt{\bar{\alpha}_{t-1}} \beta_t}{1-\bar{\alpha}_t} \hat{\mathbf{x}}_0+\frac{\sqrt{\alpha_t}\left(1-\bar{\alpha}_{t-1}\right)}{1-\bar{\alpha}_t} \mathbf{x}_t$, $\alpha_t=1-\beta_t$ and $\tilde{\beta}_t:=\frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t} \beta_t$. 

In order to control the randomness of the DDPM \citep{ho2020denoising} sampling process, DDIM \citep{song2020denoising} modifies the denoising Eq.\ref{reverse} into the following form:
\label{sec:related}

\begin{equation}
\label{ddim}
\begin{aligned}
\mathbf{x}_{t-1}=\sqrt{\alpha_{t-1}} \underbrace{\left(\frac{\mathbf{x}_t-\sqrt{1-\alpha_t} \epsilon_\theta\left(\mathbf{x}_t\right)}{\sqrt{\alpha_t}}\right)}_{\text {"predicted } \mathbf{x}_0 \text { " }} 
+\underbrace{\sqrt{1-\alpha_{t-1}-\sigma_t^2} \cdot \epsilon_\theta\left(\mathbf{x}_t\right)}_{\text {"direction pointing to } \mathbf{x}_t \text { " }}+\underbrace{\sigma_t \epsilon_t}_{\text {random noise }}.
\end{aligned}
\end{equation}
By manipulating the value of $\sigma_t \in [0,1]$, the randomness of the sampling process can be controlled. When $\sigma_t=0$, the sampling process becomes a deterministic process.

\subsection{Classifier Guidance} 
\zl{in this section, the step-wise noise is set to $x_t$, but in sec.3 they are set to $z_t$.}
From the perspective of score matching \citep{vincent2011connection}, the unconditional neural network $\epsilon_\theta\left(\mathbf{x}_t; t \right)$ optimized by the diffusion models is used to predict the score function $\nabla_{\mathbf{x}_t} \log p\left(\mathbf{x}_t \right)$.
In order to more explicitly control the amount of weight the model gives to the conditioning information, \citep{dhariwal2021diffusion} proposed classifier guidance, where the diffusion score $\epsilon_\theta\left(\mathbf{x}_t; t\right)$ is modified to include the gradient of the log likelihood of an auxiliary classifier model $p_c\left(\mathbf{y} \mid \mathbf{x}_t\right)$ as follows:
\begin{equation}
\label{classifier}
\hat{\epsilon}_t=\epsilon_\theta\left(\mathbf{x}_t; t \right)-s \sigma_t \nabla_{\mathbf{x}_t} \log p_c\left(\mathbf{y} \mid \mathbf{x}_t\right),
\end{equation}
where $s$ is employed to modulate the gradient magnitude of the noisy classifier, thereby adjusting the degree to which the model is encouraged or discouraged from considering the conditioning information.
The classifier model can also be replaced with a similarity score from a CLIP \citep{radford2021learning} model for text-to-image generation \citep{nichol2021glide}, or an arbitrary time-independent energy as in universal guidance \citep{bansal2023universal}. A recent method named self-guidance~\cite{self-guidance} proposes to convert the editing signal into gradients to replace the classifier model in diffusion sampling process. By combining this approach with classifier-free guidance \citep{ho2022classifier} as follows, self-guidance achieves high-quality results in editing the location, size and shape of the generate objects. 

\begin{equation}
\label{eq:combine}
\hat{\epsilon}_t=(1+s) \epsilon_\theta\left(\mathbf{x}_t ; t, \mathbf{y}\right)-s \epsilon_\theta\left(\mathbf{x}_t ; t, \varnothing\right)+v \sigma_t \nabla_{\mathbf{x}_t} g\left(\mathbf{x}_t ; t, \mathbf{y}\right)
\end{equation}
\zl{where ...}. In this paper, we aim to design an effective energy function to form a training-free pipeline for text-guided inpainting. 

\iffalse
classifier-free sampling \citep{ho2022classifier}
\begin{equation}
\label{classifier-free}
\hat{\epsilon}_t=(1+s) \epsilon_\theta\left(\mathbf{x}_t ; t, y\right)-s \epsilon_\theta\left(\mathbf{x}_t ; t, \varnothing\right)
\end{equation}
\fi

\iffalse
\subsection{Latent Diffusion Models}
Due to the extensive computational resources required for diffusion and denoising directly at the image level, \cite{rombach2022high} introduces latent diffusion model. Latent diffusion model employs an encoder to map images to a feature space $\mathbf{z}_0=\mathcal{E}(\mathbf{x}_0)$, then utilizes a decoder to map them back to the image space $\mathcal{D}(\mathbf{z}_0) \approx I$, while training a diffusion model in the feature space to predict the Gaussian noise added during the forward process. The most renowned latent diffusion model is Stable Diffusion \citep{rombach2022high}, which is a large-scale text-to-image generation model. Due to the high quality of text-to-image generation provided by Stable Diffusion, we implement our method in conjunction with Stable Diffusion.
\fi

\iffalse
\subsection{Image Editing}
discuss editing methods based on the attention of t2i generative methods. such as prompt2prompt, self guidance, dragondiffusion etc.
\fi

\iffalse
\subsection{Image Editing}
%Prompt2Prompt \citep{hertz2022prompt} discovered that cross-attention layers are crucial for controlling image with text. Based on their observations, they develop several image editing applications that use textual prompts for editing, such as localized editing by replacing a word, global editing by adding a specification, and controlling the extent to which a word is reflected in the image.
Recent works have used pretrained text-to-image diffusion models for image editing, Prompt2Prompt \citep{hertz2022prompt} accomplishes targeted object editing by establishing a correspondence between textual features and intermediate features within the image. SDEdit \citep{meng2021sdedit} conducts image editing by introducing noise to the original image and subsequently denoising it under new textual conditions. InstructionP2P \citep{brooks2023instructpix2pix} achieves image editing by fine-tuning the model while utilizing text as a guiding instruction for the editing process. 
\fi


\subsection{image inpainting} 
%Image inpainting is a critical task, which aims to remove undesired pixels or regions within images and replace them with visually coherent and semantically plausible content. 
%This task typically involves the use of binary masks to identify the areas that need to be erased and subsequently filled. The primary objective of image inpainting is to generate an output image that retains the overall structure and appearance of the original image while seamlessly incorporating the synthesized content in the masked regions. 
Recently, Diffusion Probabilistic Models have received increasing attention due to their impressive ability in image generation.
In the task of image inpainting, \cite{lugmayr2022repaint}  has already demonstrated that unconditional generative models are capable of inpainting images through a repainting process, which modifies the denoising process to condition generation on the unerased image content. \citep{xie2023smartbrush} \zl{discuss more methods including gan based and diffusion based methods.}

The work most closely related to ours is Inst-Inpaint \citep{yildirim2023inst}, which also removes objects from images based on textual descriptions. However, unlike our method, Inst-Inpaint first requires segmenting images based on prompts and then using diffusion models to fill in the segmented mask areas. Additionally, Inst-Inpaint requires the provision of masks for object annotation during the training phase. As a result, it is still unable to perform inpainting on objects that are difficult to annotate with masks, and it cannot preserve background information when inpainting semi-transparent objects.


